Alea Iacta Est: Auctions, Persuasion, Interim Rules, and Dice

To select a subset of samples or "winners" from a population of candidates, order sampling [Rosen 1997] and the k-unit Myerson auction [Myerson 1981] share a common scheme: assign a (random) score to each candidate, then select the k candidates with the highest scores. We study a generalization of both order sampling and Myerson's allocation rule, called winner-selecting dice. The setting for winner-selecting dice is similar to auctions with feasibility constraints: candidates have random types drawn from independent prior distributions, and the winner set must be feasible subject to certain constraints. Dice (distributions over scores) are assigned to each type, and winners are selected to maximize the sum of the dice rolls, subject to the feasibility constraints. We examine the existence of winner-selecting dice that implement prescribed probabilities of winning (i.e., an interim rule) for all types. Our first result shows that when the feasibility constraint is a matroid, then for any feasible interim rule, there always exist winner-selecting dice that implement it. Unfortunately, our proof does not yield an efficient algorithm for constructing the dice. In the special case of a 1-uniform matroid, i.e., only one winner can be selected, we give an efficient algorithm that constructs winner-selecting dice for any feasible interim rule. Furthermore, when the types of the candidates are drawn in an i.i.d.~manner and the interim rule is symmetric across candidates, unsurprisingly, an algorithm can efficiently construct symmetric dice that only depend on the type but not the identity of the candidate.

==> appendthm.tex <==
\section{Theorem B.11 of \cite{lasserre2010moments}}
\label{sec:appendthm}
The theorem is a generalization of the fundamental theorem of linear programming to uncountable dimensions. 
\begin{theorem}
  Let $f_1, \dots, f_m : \mathbb{X} \to \mathbb{R}$ be Borel measurable on a measurable space $\mathbb{X}$ and let $\mu$ be a probability measure on $\mathbb{X}$ such that $f_i$ is integrable with respect to $\mu$ for each $i=1,\dots, m$.  Then there exists a probability measure $\varphi$ with finite support on $\mathbb{X}$, such that:
\[\int_{\mathbb{X}} f_id\varphi = \int_{\mathbb{X}} f_id\mu, \quad \forall i=1, \dots, m. \]

Moreover, the support of $\varphi$ may consist of at most $m+1$ points. 
\end{theorem}

